Transverse oscillations of loops with coronal rain observed by Hinode/SOT

The condensations composing coronal rain, falling down along loop-like structures observed in cool chromospheric lines such as H$\alpha$ and \ion{Ca}{2} H, have long been a spectacular phenomenon of the solar corona. However, considered a peculiar sporadic phenomenon, it has not received much attention. This picture is rapidly changing due to recent high resolution observations with instruments such as \textit{Hinode}/SOT, CRISP of \textit{SST} and \textit{SDO}. Furthermore, numerical simulations have shown that coronal rain is a loss of thermal equilibrium of loops linked to footpoint heating. This result has highlighted the importance that coronal rain can play in the field of coronal heating. In this work, we further stress the importance of coronal rain by showing the role it can play in the understanding of the coronal magnetic field topology. We analyze \textit{Hinode}/SOT observations in the \ion{Ca}{2} H line of a loop in which coronal rain puts in evidence in-phase transverse oscillations of multiple strand-like structures. The periods, amplitudes, transverse velocities and phase velocities are calculated, allowing an estimation of the energy flux of the wave and the coronal magnetic field inside the loop through means of coronal seismology. We discuss the possible interpretations of the wave as either standing or propagating torsional Alfv\'en or fast kink waves. An estimate of the plasma beta parameter of the condensations indicates a condition that may allow the often observed separation and elongation processes of the condensations. We also show that the wave pressure from the transverse wave can be responsible for the observed low downward acceleration of coronal rain.

==> table1.tex <==
\ProvidesFile{table1.tex}%
 [2003/12/12 5.2/AAS markup document class]%
 
\begin{deluxetable}{cccc}
\tabletypesize{}
%\rotate
\tablecaption{Oscillation features for the events}
\tablewidth{0pt}
\tablehead{
\colhead{Events} & \colhead{Period} & \colhead{Amplitude} & \colhead{Transversal} \\
 & \colhead{[s]} & \colhead{[km]} & \colhead{velocity [km/s]}
}
\startdata
1 & 112 $\pm$ 29 & 245 $\pm$ 148 &  4.5 $\pm$ 2.5\\
2 & 171 $\pm$ 11 & 515 $\pm$ 135 &  6.1 $\pm$ 1.4\\
3 & 118 $\pm$ 15 & 308 $\pm$ 136 &  5.3 $\pm$ 1.3\\
4 & 143 $\pm$ 17 & 324 $\pm$ 125 &  4.4 $\pm$ 1.2\\
5 & 165 $\pm$ - & 351 $\pm$ 55 &  4.2 $\pm$ 0.1\\
6 & 198 $\pm$ 49 & 371 $\pm$ 205 &  3.6 $\pm$ 2.0\\
%7 & 172 $\pm$ 20 & 406 $\pm$ 179 &  4.2 $\pm$ 1.0\\
7 & 176 $\pm$ 23 & 369 $\pm$ 255 &  3.8 $\pm$ 2.7\\
8 & 84 $\pm$ 8 & 305 $\pm$ 119 & 7.6 $\pm$ 4.0 \\
\enddata
\tablecomments{Periods, amplitudes and transversal velocities with respective standard deviations for the 8 detected oscillatory events. Since event 5 is only observed to oscillate through 1 period before fading out, the calculation of the standard deviation is not possible for this case.  \label{table1}}
\end{deluxetable}

\endinput


==> table2.tex <==
\ProvidesFile{table2.tex}%
 [2003/12/12 5.2/AAS markup document class]%
 
\begin{deluxetable}{cccc}
\tabletypesize{}
%\rotate
\tablecaption{Wave properties and magnetic field}
\tablewidth{0pt}
\tablehead{
\colhead{Events} & \colhead{Phase speed} & \colhead{Magnetic field} & \colhead{Magnetic field} \\
 & \colhead{[km s$^{-1}$]} & \colhead{[G] ($\rho_{e}=\rho_{0}$)} & \colhead{[G] ($\rho_{e}=0$)}
}
\startdata
1 & 761 $\pm$ 264 & 21.5 $\pm$ 7.5 &  15.2 $\pm$ 5.3\\
2 & 461 $\pm$ 30 & 13 $\pm$ 0.8 &  9.2 $\pm$ 0.6\\
3 & 677 $\pm$ 89 & 19 $\pm$ 2.5 &  13.5 $\pm$ 1.8\\
4 & 555 $\pm$ 67 & 15.7 $\pm$ 1.9 &  11.1 $\pm$ 1.3\\
5 & 476 $\pm$ - & 13.5 $\pm$ - &  9.5 $\pm$ - \\
6 & 411 $\pm$ 91 & 11.6 $\pm$ 2.5 &  8.2 $\pm$ 1.9\\
%7 & 460 $\pm$ 58 & 0.48$\pm$0.21 & 13 $\pm$ 1.6 &  9.2 $\pm$ 1.2\\
7 & 452 $\pm$ 60 & 12.8 $\pm$ 1.7 &  9 $\pm$ 1.2\\
8 & 942 $\pm$ 96 & 26.7 $\pm$ 2.7 & 18.8 $\pm$ 1.9 \\
\enddata
\tablecomments{Average phase speeds, energy fluxes and magnetic fields for each oscillation event in Table~\ref{table1}, with the corresponding standard deviations. The magnetic fields are calculated according to Equation \ref{Bkink} for two limiting cases:  an exterior to interior density ratio of 1 (\textit{third column}), or a density ratio of 0 (\textit{fourth column}).   \label{table2}}
\end{deluxetable}

\endinput

